UniDemoir\'e: Towards Universal Image Demoir\'eing with Data Generation and Synthesis

Image demoir\'eing poses one of the most formidable challenges in image restoration, primarily due to the unpredictable and anisotropic nature of moir\'e patterns. Limited by the quantity and diversity of training data, current methods tend to overfit to a single moir\'e domain, resulting in performance degradation for new domains and restricting their robustness in real-world applications. In this paper, we propose a universal image demoir\'eing solution, UniDemoir\'e, which has superior generalization capability. Notably, we propose innovative and effective data generation and synthesis methods that can automatically provide vast high-quality moir\'e images to train a universal demoir\'eing model. Our extensive experiments demonstrate the cutting-edge performance and broad potential of our approach for generalized image demoir\'eing.

==> Tables/tbl_datasets_mobile_phone.tex <==
\begin{table}[h]
\centering
\caption{The mobile phone we apply to get the moiré patterns}
% \begin{subtable}{0.5\linewidth}
\vspace{-0.5ex}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
Mobile Phone & Camera & CMOS & MegaPixel ($\text{MP}$) \\
\midrule
\multirow{1}{*}{iPhone 12}     & Main      & SONY   IMX503            & 12   \\
%\hline
\multirow{1}{*}{iPhone 13}     & Main      & SONY IMX603              & 12   \\
%\hline
\multirow{1}{*}{Honor 90}      & Main      & ISOCELL HP3              & 200  \\
%\hline
\multirow{1}{*}{Xiaomi 10s}    & Main      & ISOCELL HMX              & 108  \\
%\hline \cline
\midrule
\multirow{2}{*}{iPhone 12 Pro} & Main      & SONY IMX503              & 12   \\
                               & Telephoto & SONY IMX613 (2x zoom)    & 12.2 \\
\midrule
\multirow{2}{*}{iPhone 15 Pro} & Main      & SONY IMX803              & 48   \\
                               % \cline{2-6}
                               & Telephoto & SONY IMX713 (2x/3x zoom) & 12   \\
\bottomrule
\end{tabular}
}
\label{tab:Datasets-Phone}
\end{table}

==> Tables/tbl_datasets_overview.tex <==
% \begin{table*}[t]
% \centering
% \caption{Comparisons of different moiré datasets. %Our datasets and MoireSpace~\cite{yang2023doing} are moiré pattern datasets, while TIP2018~\cite{sun2018moire}, LCDMoiré~\cite{yuan2019aim}, FHDMi~\cite{he2020fhde} and UHDM~\cite{yu2022towards} are demoiréing datasets with paired moiré images
% }

% \scalebox{0.775}{
% \begin{tabular}{ccc|ccccccc}
% \toprule
% \multicolumn{3}{c|}{Datasets} & \multirow{2.5}{*}{Avg. Resolution} & \multirow{2.5}{*}{Size} & \multicolumn{5}{c}{Capture settings}   \\ 
% \cmidrule{1-3} \cmidrule{6-10} 
% \multicolumn{2}{c}{Type} & Name &       &      & Phone  & Screen & Multiple zooming rate & Multiple camera / CMOS  & Screen Panel \\ 
% \midrule
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} Moiré Image \\ Dataset\end{tabular}}  
% % TIP2018$_{\text{Real}}$
% & Real      & TIP2018(Real) & 256 $\times$ 256   & 135000 & 3     & 3      & \ding{55}(1x-only) & \ding{55}(Main-only) & IPS-only     \\
% & Real      & FHDMi     & 1024 $\times$ 1024 & 12000  & 3     & 2      & \ding{55}(1x-only) & \ding{55}(Main-only) & IPS-only     \\
% & Real      & UHDM   & 4328 $\times$ 3248 & 4500   & 3     & 3      & \ding{55}(1x-only) & \ding{55}(Main-only) & IPS-only     \\ 
% & Synthetic & LCDMoiré & 1024 $\times$ 1024 & 10200  & -     & -      & -          & -            & -            \\ 
% \midrule

% \multirow{2.5}{*}{\begin{tabular}[c]{@{}c@{}} Moiré Pattern \\ Dataset\end{tabular}} 
% & Real & MoireSpace  & 2160 $\times$ 1286 & 18147  & 3     & 3      & \ding{55}(1x-only) & \ding{55}(Main-only) & IPS-only     \\ \cmidrule{2-10}
% & \cellcolor{Gray}\textbf{Real} & \cellcolor{Gray}\textbf{Ours}       
% & \cellcolor{Gray}\textbf{3840} $\times$ \textbf{2160} & \cellcolor{Gray}\textbf{150000} & \cellcolor{Gray}\textbf{6} & \cellcolor{Gray}\textbf{6} 
% & \cellcolor{Gray}\textbf{\checkmark(1x,2x,3x)} & \cellcolor{Gray}\textbf{\checkmark(Main,Telephoto)} & \cellcolor{Gray}\textbf{IPS, SVA}  \\ 

% \bottomrule
% \end{tabular}
% }
% \label{tab:datasets-overview}
% \end{table*}


\begin{table*}[ht]
\centering
\small
\setlength{\tabcolsep}{2.85mm}

% \scalebox{0.8}{
% \begin{tabular}{c @{\hskip +2em} c@{\hskip +2em} |c@{\hskip +2em}c@{\hskip +2em}  c@{\hskip +2em} c@{\hskip +2em} c@{\hskip +2em} c@{\hskip +2em} c}

\scalebox{0.85}{
\begin{tabular}{cc|ccccccc}

\toprule[1.25pt]
\multicolumn{2}{c|}{Datasets} & \multirow{2.5}{*}{Avg. Resolution} & \multirow{2.5}{*}{Size} & \multicolumn{5}{c}{Capture settings}   \\ 
\cmidrule(lr){1-2} \cmidrule(lr){5-9} 
Type & Name &       &      & Phone  & Screen & Multi-zooming rate & Multi-camera / CMOS  & Screen Panel \\ 
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} Moiré Image \\ Dataset\end{tabular}}  
% TIP2018$_{\text{Real}}$
% 
& TIP2018(R) & 256 $\times$ 256   & 135000 & 3     & 3      & \ding{55}(1x-only) & \ding{55}(Main-only) & IPS-only     \\
& FHDMi(R)     & 1024 $\times$ 1024 & 12000  & 3     & 2      & \ding{55}(1x-only) & \ding{55}(Main-only) & IPS-only     \\
& UHDM(R)   & 4328 $\times$ 3248 & 5000   & 3     & 3      & \ding{55}(1x-only) & \ding{55}(Main-only) & IPS-only     \\ 
& LCDMoiré(S) & 1024 $\times$ 1024 & 10200  & -     & -      & -          & -            & -            \\ 
\midrule

\multirow{2.5}{*}{\begin{tabular}[c]{@{}c@{}} Moiré Pattern \\ Dataset\end{tabular}} 
& MoireSpace(R)  & 2160 $\times$ 1286 & 18147  & 3     & 3      & \ding{55}(1x-only) & \ding{55}(Main-only) & IPS-only     \\ 
\cmidrule{2-9}
& \textbf{Ours(R)} & \textbf{3840} $\times$ \textbf{2160} & \textbf{150000} & \textbf{6} & \textbf{6} & \textbf{\checkmark(1x,2x,3x)} & \textbf{\checkmark(Main,Telephoto)} & \textbf{IPS, SVA}  \\ 

\bottomrule[1.25pt]
\end{tabular}
}
\caption{Comparisons of different moiré datasets. The ``R'' denotes the real dataset, and the ``S'' denotes the synthetic dataset. %Our datasets and MoireSpace~\cite{yang2023doing} are moiré pattern udatasets, while TIP2018~\cite{sun2018moire}, LCDMoiré~\cite{yuan2019aim}, FHDMi~\cite{he2020fhde} and UHDM~\cite{yu2022towards} are demoiréing datasets with paired moiré images
}
\vspace{-1ex}
\label{tab:datasets-overview}
\end{table*}

==> Tables/tbl_exp_ablation.tex <==

% \begin{table}[h]
% \centering
% \setlength{\tabcolsep}{2.5mm}
% \scalebox{0.9}{
% \begin{tabular}{lccc}
% \toprule
% \multirow{2.5}{*}{Components}  & \multicolumn{3}{c}{Test set: FHDMi}  \\ 
%                              \cmidrule(l){2-4} 
%                              &\ua{PSNR }   &\ua{SSIM } &\da{LPIPS } \\ 
% \midrule
% \multicolumn{4}{l}{\textit{Using:   \textbf{ESDNet-L}, trained with \textbf{UHDM}, 50 Epochs}} \\ 
% \midrule
% ALL                          & \textbf{12.3456} & \textbf{0.1234} & \textbf{0.1234} \\
% $w/o$ MPG                    &                  &                 &                 \\
% $w/o$ TRN                    &                  &                 &                 \\
% TRN ($w/o$ $\mathcal{L}_{per}$)    &                  &                 &                 \\
% TRN ($w/o$ $\mathcal{L}_{color}$)  &                  &                 &                 \\
% TRN ($w/o$ $\mathcal{L}_{tv}$)     &                  &                 &                 \\
% TRN ($w/o$ fusion block)           &                  &                 &                 \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation studies. UHDM is the source dataset for training, while FHDMi is the target dataset for testing.}
% \label{tab:Exp_ablation}
% \end{table}


\begin{table}[h]
\centering
\setlength{\tabcolsep}{2.8mm}
\scalebox{0.8}{
\begin{tabular}{l  @{\hskip +3em} c  @{\hskip +3em} c  @{\hskip +3em} c}
%\scalebox{0.9}{
%\begin{tabular}{lccc}
\toprule
% \multirow{2.5}{*}{Components}  & \multicolumn{3}{c}{Test set: FHDMi}  \\ \cmidrule(l){2-4} 
Components                     &\ua{PSNR}   &\ua{SSIM} &\da{LPIPS} \\ 
% \midrule
% \multicolumn{4}{l}{\textit{Using:   \textbf{ESDNet-L}, trained with \textbf{UHDM}, 50 Epochs}} \\ 
\midrule
ALL                          & \textbf{20.7543} & \textbf{0.7653} & \textbf{0.2136} \\

$w/o$ MPG                    & 20.1607          & 0.7326          & 0.2456          \\
$w/o$ TRN                    & 20.1691          & 0.7372          & 0.2544          \\
TRN ($w/o$ $\mathcal{L}_{per}$)    & 20.3076          & 0.7508          & 0.2558          \\
TRN ($w/o$ $\mathcal{L}_{color}$)  & 20.2692          & 0.7406          & 0.2301          \\
TRN ($w/o$ $\mathcal{L}_{tv}$)     & 20.3961          & 0.7451          & 0.2324          \\
TRN ($w/o$ fusion block)           & 20.2868          & 0.7370          & 0.2311          \\ 
\bottomrule
\end{tabular}
}
\caption{Ablation studies. Source: UHDM, Target: FHDMi.}
\vspace{-2.5ex}
\label{tab:Exp_ablation}
\end{table}

		
		
		
		
		
	  	



==> Tables/tbl_exp_cross_datasets.tex <==
% \begin{table}[t]

% % Demoireing results on the UHDM dataset training with synthesized data only. 
% % Since both our method and shooting~\cite{shooting} borrow none real moire patterns in dataset UHDM, for fairness, we instruct UnDem~\cite{undem} to utilize the moire patterns from FHDMi. Method "Paired" indicates training using the original real moire data in the training set of UHDM.
% % The "C.S." denotes size in the random crop. $(\uparrow)$ denotes the larger, the better, and $(\downarrow)$ denotes the smaller, the better.
% \caption{Cross-dataset Evaluations %The ``Paired'' indicates training demoiréing network using paired data from the source dataset, and the ``UnDeM'' indicates training demoiréing network using pseudo-paired data generated by the GAN-based generator trained on the source dataset.
% }
% \centering
% \newcolumntype{g}{>{\columncolor{Gray}}c}
% % \renewcommand\tabcolsep{5.0pt}
% % \vspace{-8pt}
% % \resizebox{10cm}{!}       % \textwidth, 10cm, 这里用 10cm 好像效果好于 \textwidth
% %\scalebox{0.85}{    
% \resizebox{.48\textwidth}{!}{
% \begin{tabular}{cccc|ccc}
% \toprule[1.25pt]    % 顶部粗线
% Model                      & Source                 & Target                 & Metric    & Original  & UnDeM   &  \textbf{Ours} \\ 
% \midrule
% \multirow{18}{*}{MBCNN}    & \multirow{6}{*}{UHDM}  & \multirow{3}{*}{FHDMi} &\ua{PSNR } & 19.3848 & 19.4676 & \textbf{20.3260} \\
%                            &                        &                        &\ua{SSIM } & 0.7536  & 0.7555  & \textbf{0.7812}  \\
%                            &                        &                        &\da{LPIPS }& 0.2902  & 0.2864  & \textbf{0.2355}  \\ 
%                            \cmidrule{3-7} 
%                            &                        & \multirow{3}{*}{TIP}   &\ua{PSNR } & 17.8107 & 19.6674 & \textbf{20.7684} \\
%                            &                        &                        &\ua{SSIM } & 0.6627  & 0.6911  & \textbf{0.7465}  \\
%                            &                        &                        &\da{LPIPS }& 0.3580  & 0.3909  & \textbf{0.2871}  \\ 
%                            \cmidrule{2-7} 
%                            & \multirow{6}{*}{FHDMi} & \multirow{3}{*}{UHDM}  &\ua{PSNR } & 17.1331 & 17.4870 & \textbf{18.2999} \\
%                            &                        &                        &\ua{SSIM } & 0.6159  & 0.6331  & \textbf{0.6772}  \\
%                            &                        &                        &\da{LPIPS }& 0.4470  & 0.4285  & \textbf{0.3822}  \\ 
%                            \cmidrule{3-7} 
%                            &                        & \multirow{3}{*}{TIP}   &\ua{PSNR } & 20.2161 & 20.8261 & \textbf{21.1324} \\
%                            &                        &                        &\ua{SSIM } & 0.7340  & 0.7381  & \textbf{0.7449}  \\
%                            &                        &                        &\da{LPIPS }& 0.2879  & 0.2791  & \textbf{0.2770}  \\ 
%                            \cmidrule{2-7} 
%                            & \multirow{6}{*}{TIP}   & \multirow{3}{*}{UHDM}  &\ua{PSNR } & 17.3409 & 17.4407 & \textbf{17.7890} \\
%                            &                        &                        &\ua{SSIM } & 0.6144  & 0.6066  & \textbf{0.6549}  \\
%                            &                        &                        &\da{LPIPS }& 0.4726  & 0.4473  & \textbf{0.4286}  \\
%                            \cmidrule{3-7}
%                            &                        & \multirow{3}{*}{FHDMi} &\ua{PSNR } & 18.9458 & 19.0336 & \textbf{19.2419} \\
%                            &                        &                        &\ua{SSIM } & 0.7369  & 0.7215  & \textbf{0.7441}  \\
%                            &                        &                        &\da{LPIPS }& 0.2494  & 0.2452  & \textbf{0.2256}  \\
% \midrule
% \midrule
% \multirow{18}{*}{ESDNet-L} & \multirow{6}{*}{UHDM}  & \multirow{3}{*}{FHDMi} &\ua{PSNR } & 20.3422 & 20.4014 & \textbf{22.0638} \\
%                            &                        &                        &\ua{SSIM } & 0.7699  & 0.7710  & \textbf{0.8021}  \\
%                            &                        &                        &\da{LPIPS }& 0.2525  & 0.2509  & \textbf{0.1707}  \\ 
%                            \cmidrule{3-7} 
%                            &                        & \multirow{3}{*}{TIP}   &\ua{PSNR } & 18.8040 & 19.3545 & \textbf{19.9983} \\
%                            &                        &                        &\ua{SSIM } & 0.6921  & 0.6998  & \textbf{0.7052}  \\
%                            &                        &                        &\da{LPIPS }& 0.3524  & 0.3601  & \textbf{0.3301}  \\ 
%                            \cmidrule{2-7} 
%                            & \multirow{6}{*}{FHDMi} & \multirow{3}{*}{UHDM}  &\ua{PSNR } & 18.0049 & 17.9574 & \textbf{18.6718} \\
%                            &                        &                        &\ua{SSIM } & 0.5755  & 0.5857  & \textbf{0.6867}  \\
%                            &                        &                        &\da{LPIPS }& 0.4420  & 0.4460  & \textbf{0.3621}  \\ 
%                            \cmidrule{3-7} 
%                            &                        & \multirow{3}{*}{TIP}   &\ua{PSNR } & 20.6647 & 20.4663 & \textbf{21.2096} \\
%                            &                        &                        &\ua{SSIM } & 0.7504  & 0.7278  & \textbf{0.7602}  \\
%                            &                        &                        &\da{LPIPS }& 0.2359  & 0.2998  & \textbf{0.2231}  \\ 
%                            \cmidrule{2-7} 
%                            & \multirow{6}{*}{TIP}   & \multirow{3}{*}{UHDM}  &\ua{PSNR } & 17.4332 & 16.8402 & \textbf{18.0582} \\
%                            &                        &                        &\ua{SSIM } & 0.5523  & 0.5692  & \textbf{0.6586}  \\
%                            &                        &                        &\da{LPIPS }& 0.4987  & 0.4532  & \textbf{0.3716}  \\ 
%                            \cmidrule{3-7} 
%                            &                        & \multirow{3}{*}{FHDMi} &\ua{PSNR } & 19.2368 & 19.2112 & \textbf{19.4041} \\
%                            &                        &                        &\ua{SSIM } & 0.7354  & 0.7499  & \textbf{0.7573}  \\
%                            &                        &                        &\da{LPIPS }& 0.2316  & 0.2130  & \textbf{0.2118}  \\ 
% \bottomrule  % 底部粗线
% \end{tabular}
% }
% \label{tab:Exp_cross_datasets}
% \end{table}





% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[t]

% \caption{Cross-dataset Evaluations}
% % \setlength{\tabcolsep}{1mm}
% % \setlength{\tabcolsep}{1mm}
% \centering
% \resizebox{.474\textwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule[1.25pt]    % 顶部粗线
% % \multirow{2}{*}{\makecell{Cross-dataset \\(Train→Test)}}
% % \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cross-dataset \\(Train→Test)\end{tabular}}
% % \makecell{Cross-dataset \\ (Train→Test)}

% \multirow{2.5}{*}{\multicolumn{1}{c}{\makecell{Cross \\ Dataset}}} & \multirow{2.5}{*}{Metric} & \multirow{2.5}{*}{Baseline} & \multicolumn{4}{c}{Moire Image Synthesis   Method} \\ 
% \cmidrule(lr){4-7} 
% &      &  
% & Shooting    & UnDeM      & MoireSpace    & Ours    \\ 
% \midrule
% \midrule
% \multicolumn{7}{c}{\textit{Demoiréing Model: \textbf{MBCNN}}}\\
% % \cmidrule(lr){3-5} 
% \midrule
% % UHDM $\rightarrow$ FHDMi 
% % UHDM \\ $\downarrow$ \\ FHDMi
% % UHDM \\  $\rightarrow$ FHDMi 
% % \begin{tabular}[c]{@{}c@{}}UHDM \\$\rightarrow$ FHDMi\end{tabular}
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}UHDM \\ $\rightarrow$ FHDMi\end{tabular}} 
% & PSNR  & 19.3848 & 19.2032 & 19.4676 &         &         \\
% & SSIM  & 0.7536  & 0.7459  & 0.7555  &         &         \\
% & LPIPS & 0.2902  & 0.2975  & 0.2864  &         &         \\
% \midrule
% % UHDM→TIP
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}UHDM \\ $\rightarrow$ TIP\end{tabular}}   
% & PSNR  & 17.8107 & 18.373  & 19.6674 &         &         \\
% & SSIM  & 0.6627  & 0.6888  & 0.6911  &         &         \\
% & LPIPS & 0.3580  & 0.3886  & 0.3909  &         &         \\
% \midrule
% % FHDMi→UHDM
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}FHDMi \\ $\rightarrow$ UHDM\end{tabular}} 
% & PSNR  & 17.1331 &         & 17.487  &         &         \\
% & SSIM  & 0.6159  &         & 0.6331  &         &         \\
% & LPIPS & 0.4470  &         & 0.4285  &         &         \\
% \midrule
% % FHDMi→TIP
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}FHDMi \\ $\rightarrow$ TIP\end{tabular}}  
% & PSNR  & 20.2161 &         & 20.8261 &         &         \\
% & SSIM  & 0.7340  &         & 0.7381  &         &         \\
% & LPIPS & 0.2879  &         & 0.2791  &         &         \\
% \midrule
% % TIP→UHDM
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}TIP \\ $\rightarrow$ UHDM\end{tabular}} 
% & PSNR  & 17.3409 &         & 17.4407 &         &         \\
% & SSIM  & 0.6144  &         & 0.6066  &         &         \\
% & LPIPS & 0.4726  &         & 0.4473  &         &         \\
% \midrule
% % TIP→FHDMi
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}TIP \\ $\rightarrow$ FHDMi\end{tabular}}
% & PSNR  & 18.9458 &         & 19.0336 &         &         \\
% & SSIM  & 0.7369  &         & 0.7215  &         &         \\
% & LPIPS & 0.2494  &         & 0.2452  &         &         \\ 
% \midrule
% \midrule
% % \textit{Demoiréing Model: \textbf{ESDNet-L}}
% % \multirow{1}{*}{\textit{Demoiréing Model: \textbf{ESDNet-L}}}
% % \multirow{0.7}{*}{\textit{Demoiréing Model: \textbf{ESDNet-L}}}
% \multicolumn{7}{c}{\textit{Demoiréing Model: \textbf{ESDNet-L}}} \\
% \midrule
% % \cmidrule{1-2}
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}UHDM \\ $\rightarrow$ FHDMi\end{tabular}}                              
% & PSNR  & 20.3422 & 20.2407 & 20.4014 &         &         \\
% & SSIM  & 0.7699  & 0.7579  & 0.771   &         &         \\
% & LPIPS & 0.2525  & 0.2632  & 0.2509  &         &         \\
% \midrule
% % UHDM→TIP
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}UHDM \\ $\rightarrow$ TIP\end{tabular}}
% & PSNR  & 18.804  & 18.4543 & 19.3545 &         &         \\
% & SSIM  & 0.6921  & 0.693   & 0.6998  &         &         \\
% & LPIPS & 0.3524  & 0.3849  & 0.3601  &         &         \\
% \midrule
% % FHDMi→UHDM
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}FHDMi \\ $\rightarrow$ UHDM\end{tabular}} 
% & PSNR  & 18.0049 &         & 17.9574 &         &         \\
% & SSIM  & 0.5755  &         & 0.5857  &         &         \\
% & LPIPS & 0.442   &         & 0.446   &         &         \\
% \midrule
% % FHDMi→TIP
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}FHDMi \\ $\rightarrow$ TIP \end{tabular}}  
% & PSNR  & 20.6647 &         & 20.4663 &         &         \\
% & SSIM  & 0.7504  &         & 0.7278  &         &         \\
% & LPIPS & 0.2359  &         & 0.2998  &         &         \\
% \midrule
% % TIP→UHDM
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}TIP \\ $\rightarrow$ UHDM\end{tabular}}  
% & PSNR  & 17.4332 &         & 16.8402 &         &         \\
% & SSIM  & 0.5523  &         & 0.5692  &         &         \\
% & LPIPS & 0.4987  &         & 0.4532  &         &         \\
% \midrule
% % TIP→FHDMi
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}TIP \\ $\rightarrow$ FHDMi\end{tabular}} 
% & PSNR  & 19.2368 &         & 19.2112 &         &         \\
% & SSIM  & 0.7354  &         & 0.7499  &         &         \\
% & LPIPS & 0.2316  &         & 0.213   &         &         \\ 
% \bottomrule[1.25pt]  % 底部粗线
% \end{tabular}
% }
% \label{tab:Exp_cross_datasets}

% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{2.3mm}
% \scalebox{0.65}{
% \begin{tabular}{c @{\hskip +3em}c@{\hskip +3em}c@{\hskip +3em}|c@{\hskip +3em}c @{\hskip +3em} c @{\hskip +3em}c @{\hskip +3em} c@{\hskip +3em}| c @{\hskip +3em}c @{\hskip +3em}c @{\hskip +3em}c @{\hskip +3em}c}
\scalebox{0.85}{
\begin{tabular}{ccc|ccccc|ccccc}
\toprule[1.25pt]    % 顶部粗线
% \multicolumn{2}{c}{\multirow{2.5}{*}{\makecell{Cross Dataset \\ Evaluations}}} & \multirow{4}{*}{Metric} & \multicolumn{5}{c|}{Demoiréing Model: \textbf{MBCNN}} & \multicolumn{5}{c}{Demoiréing Model: \textbf{ESDNet-L}} \\ 
% \cmidrule(lr){4-8} \cmidrule(lr){9-13} 
% \multicolumn{2}{c}{} &     & \multirow{2}{*}{Baseline} & \multicolumn{4}{c|}{Moiré Image Synthesis Method} & \multirow{2}{*}{Baseline} & \multicolumn{4}{c}{Moiré Image Synthesis Method} \\ 
% \cmidrule(lr){1-2} \cmidrule(lr){5-8} \cmidrule(lr){10-13} 

% \multicolumn{1}{c}{Cross Dataset} & \multirow{2.5}{*}{Metric} & \multicolumn{5}{c|}{Demoiréing Model: \textbf{MBCNN}} & \multicolumn{5}{c}{Demoiréing Model: \textbf{ESDNet-L}} \\ 
% \cmidrule(lr){4-8} \cmidrule(lr){9-13} 
% \multicolumn{2}{c}{} &     & \multirow{2}{*}{Baseline} & \multicolumn{4}{c|}{Moiré Image Synthesis Method} & \multirow{2}{*}{Baseline} & \multicolumn{4}{c}{Moiré Image Synthesis Method} \\ 
% \cmidrule(lr){1-2} \cmidrule(lr){5-8} \cmidrule(lr){10-13} 

\multicolumn{2}{c}{Cross Dataset}& \multirow{2.5}{*}{Metric} & \multicolumn{5}{c|}{Demoiréing Network: \textbf{MBCNN}}  & \multicolumn{5}{c}{Demoiréing Network:   \textbf{ESDNet-L}}  \\ 
\cmidrule(lr){1-2} \cmidrule(lr){4-8}  \cmidrule(lr){9-13}

Source & Target &        & Baseline & Shooting & UnDeM & MoireSpace & Ours  & Baseline & Shooting & UnDeM & MoireSpace   & Ours   \\ 
\midrule
\midrule
\multirow{6.5}{*}{UHDM}    
& \multirow{3}{*}{FHDMi} &\ua{PSNR } & 19.3848 & 19.2032 & 19.4676 & 19.4531 & \textbf{19.8625} & 20.3422 & 20.2407 & 20.4014 & 20.2806 & \textbf{20.7543} \\
&                        &\ua{SSIM } & 0.7436  & 0.7459  & 0.7455  & 0.7496  & \textbf{0.7525}  & 0.7599  & 0.7579  & 0.7510  & 0.7603  & \textbf{0.7653}  \\
&                        &\da{LPIPS }& 0.3002  & 0.2975  & 0.2964  & 0.2993  & \textbf{0.2842}  & 0.2525  & 0.2632  & 0.2509  & 0.2324  & \textbf{0.2136}  \\ 
\cmidrule{2-13} 
& \multirow{3}{*}{TIP}   &\ua{PSNR } & 17.8107 & 18.3730 & 18.6674 & 18.9214 & \textbf{19.3922} & 18.8040 & 18.4543 & 19.3545 & 19.3964 & \textbf{19.5009} \\
&                        &\ua{SSIM } & 0.6627  & 0.6888  & 0.6911  & 0.6996  & \textbf{0.7022}  & 0.6921  & 0.6930  & 0.6998  & 0.7111  & \textbf{0.7149}  \\
&                        &\da{LPIPS }& 0.3580  & 0.3886  & 0.3909  & 0.3829  & \textbf{0.3781}  & 0.3524  & 0.3849  & 0.3601  & 0.3522  & \textbf{0.3495}  \\ 
\midrule
\multirow{6.5}{*}{FHDMi}   
& \multirow{3}{*}{UHDM}  &\ua{PSNR } & 17.1331 & 17.5326 & 17.4870 & 17.6050 & \textbf{18.7931} & 18.0049 & 18.4189 & 17.9574 & 17.9751 & \textbf{18.9240} \\
&                        &\ua{SSIM } & 0.6159  & 0.6334  & 0.6331  & 0.6642  & \textbf{0.7186}  & 0.5755  & 0.5780  & 0.5857  & 0.5548  & \textbf{0.6658}  \\
&                        &\da{LPIPS }& 0.4470  & 0.4350  & 0.4285  & 0.4020  & \textbf{0.3508}  & 0.4420  & 0.4279  & 0.4460  & 0.4579  & \textbf{0.3405}  \\ 
\cmidrule{2-13} 
& \multirow{3}{*}{TIP}   &\ua{PSNR } & 20.2161 & 20.7793 & 20.8261 & 20.1194 & \textbf{21.0694} & 20.6647 & 20.8678 & 20.4663 & 20.8107 & \textbf{21.5786} \\
&                        &\ua{SSIM } & 0.7340  & 0.7304  & 0.7381  & 0.7347  & \textbf{0.7494}  & 0.7504  & 0.7606  & 0.7278  & 0.7582  & \textbf{0.7668}  \\
&                        &\da{LPIPS }& 0.2979  & 0.2884  & 0.2891  & 0.2961  & \textbf{0.2832}  & 0.2459  & 0.2450  & 0.2998  & 0.2468  & \textbf{0.2310}  \\ 
\midrule
\multirow{6.5}{*}{TIP}     
& \multirow{3}{*}{UHDM}  &\ua{PSNR } & 17.3409 & 17.4011 & 17.4407 & 17.4987 & \textbf{18.2937} & 17.4332 & 16.1836 & 16.8402 & 16.6296 & \textbf{18.4978} \\
&                        &\ua{SSIM } & 0.6144  & 0.6062  & 0.6066  & 0.6059  & \textbf{0.6913}  & 0.5523  & 0.5511  & 0.5692  & 0.5748  & \textbf{0.6866}  \\
&                        &\da{LPIPS }& 0.4726  & 0.4487  & 0.4473  & 0.4412  & \textbf{0.3990}  & 0.4987  & 0.4723  & 0.4532  & 0.4387  & \textbf{0.3231}  \\ 
\cmidrule{2-13} 
& \multirow{3}{*}{FHDMi} &\ua{PSNR } & 18.9458 & 19.2731 & 19.0336 & 19.1101 & \textbf{20.1053} & 19.2368 & 18.1936 & 19.2112 & 18.8385 & \textbf{19.9971} \\
&                        &\ua{SSIM } & 0.7369  & 0.7399  & 0.7215  & 0.7321  & \textbf{0.7725}  & 0.7354  & 0.7297  & 0.7499  & 0.7389  & \textbf{0.7580}  \\
&                        &\da{LPIPS }& 0.2494  & 0.2447  & 0.2452  & 0.2382  & \textbf{0.2315}  & 0.2316  & 0.2320  & 0.2130  & 0.2228  & \textbf{0.1915}  \\ 
\bottomrule[1.25pt]  % 底部粗线
\end{tabular}
}
\caption{Quantitative results of cross-dataset evaluations.}
\vspace{-2ex}
\label{tab:Exp_cross_datasets}
\end{table*}




















































































==> Tables/tbl_exp_cross_datasets_esdnet.tex <==
\begin{table}[t]
\caption{Cross-dataset demoireing results using ESDNet-L~\cite{yu2022towards}. The "Paired" indicates training demoireing network using paired data from the source dataset, and the "UnDeM" indicates training demoireing network using pseudo-paired data generated by the GAN-based generator trained on the source dataset. Note that $(\uparrow)$ denotes the larger, the better, and $(\downarrow)$ denotes the smaller, the better.}
\centering
\renewcommand\tabcolsep{5.0pt}
\vspace{-8pt}
% \resizebox{10cm}{!}       % \textwidth, 10cm, 这里用 10cm 好像效果好于 \textwidth
\scalebox{0.9}
{       
\begin{tabular}{ccc|ccc}
\toprule[1.2pt]    % 顶部粗线
\multirow{2}{*}{Source} & \multirow{2}{*}{Target} & \multirow{2}{*}{Metric} & \multicolumn{3}{c}{ESDNet-L~\cite{yu2022towards}}              \\ \cline{4-6} 
                        &                         &                         & Paired  & UnDeM   & Ours                     \\ \hline
\multirow{6}{*}{UHDM}   & \multirow{3}{*}{FHDMi}  & \ua{PSNR }              & 20.3422 & 17.3647 &                          \\
                        &                         & \ua{SSIM }              & 0.7699  & 0.6963  &                          \\
                        &                         & \da{LPIPS }             & 0.2525  & 0.3063  &                          \\ \cline{2-6} 
                        & \multirow{3}{*}{TIP}    & \ua{PSNR }              & 18.8040 & 17.3647 &                          \\
                        &                         & \ua{SSIM }              & 0.6921  & 0.6665  &                          \\
                        &                         & \da{LPIPS }             & 0.3524  & 0.3710  &                          \\ \hline
\multirow{6}{*}{FHDMI}  & \multirow{3}{*}{UHDM}   & \ua{PSNR }              & 18.0049 & 16.3763 &                          \\
                        &                         & \ua{SSIM }              & 0.5755  & 0.5193  &                          \\
                        &                         & \da{LPIPS }             & 0.4420  & 0.5560  &                          \\ \cline{2-6} 
                        & \multirow{3}{*}{TIP}    & \ua{PSNR }              &         & 19.1417 &                          \\
                        &                         & \ua{SSIM }              &         & 0.7178  &                          \\
                        &                         & \da{LPIPS }             &         & 0.2600  &                          \\ \hline
\multirow{6}{*}{TIP}    & \multirow{3}{*}{UHDM}   & \ua{PSNR }              & 17.4332 & -       &                          \\
                        &                         & \ua{SSIM }              & 0.5523  & -       &                          \\
                        &                         & \da{LPIPS }             & 0.4987  & -       &                          \\ \cline{2-6} 
                        & \multirow{3}{*}{FHDMi}  & \ua{PSNR }              & 19.2368 & -       &                          \\
                        &                         & \ua{SSIM }              & 0.7354  & -       &                          \\
                        &                         & \da{LPIPS }             & 0.2316  & -       &                          \\ 
\bottomrule[1.2pt]  % 底部粗线
\end{tabular}
}
\label{tab:Exp_cross_datasets_esdnet}
\end{table}



==> Tables/tbl_exp_cross_datasets_mbcnn.tex <==
\begin{table}[t]

% Demoireing results on the UHDM dataset training with synthesized data only. 
% Since both our method and shooting~\cite{shooting} borrow none real moire patterns in dataset UHDM, for fairness, we instruct UnDem~\cite{undem} to utilize the moire patterns from FHDMi~\cite{he2020fhde}. Method "Paired" indicates training using the original real moire data in the training set of UHDM.
% The "C.S." denotes size in the random crop. $(\uparrow)$ denotes the larger, the better, and $(\downarrow)$ denotes the smaller, the better.
\caption{Cross-dataset demoireing results using MBCNN. The "Paired" indicates training demoireing network using paired data from the source dataset, and the "UnDeM" indicates training demoireing network using pseudo-paired data generated by the GAN-based generator trained on the source dataset. Note that $(\uparrow)$ denotes the larger, the better, and $(\downarrow)$ denotes the smaller, the better.}
\centering
\renewcommand\tabcolsep{5.0pt}
\vspace{-8pt}
% \resizebox{10cm}{!}       % \textwidth, 10cm, 这里用 10cm 好像效果好于 \textwidth
\scalebox{0.9}
{       
\begin{tabular}{ccc|ccc}
\toprule[1.2pt]    % 顶部粗线
\multirow{2}{*}{Source} & \multirow{2}{*}{Target} & \multirow{2}{*}{Metric} & \multicolumn{3}{c}{MBCNN}              \\ \cline{4-6} 
                        &                         &                         & Paired  & UnDeM & Ours                       \\ \hline
\multirow{6}{*}{UHDM}   & \multirow{3}{*}{FHDMi}  & \ua{PSNR }              & 19.3848 & 18.1873 &                          \\
                        &                         & \ua{SSIM }              & 0.7536  & 0.7143  &                          \\
                        &                         & \da{LPIPS }             & 0.2902  & 0.2920  &                          \\ \cline{2-6} 
                        & \multirow{3}{*}{TIP}    & \ua{PSNR }              & 17.8107 & 18.6846 &                          \\
                        &                         & \ua{SSIM }              & 0.6627  & 0.6890  &                          \\
                        &                         & \da{LPIPS }             & 0.3580  & 0.3665  &                          \\ \hline
\multirow{6}{*}{FHDMI}  & \multirow{3}{*}{UHDM}   & \ua{PSNR }              &         & 17.1348 &                          \\
                        &                         & \ua{SSIM }              &         & 0.6110  &                          \\
                        &                         & \da{LPIPS }             &         & 0.4277  &                          \\ \cline{2-6} 
                        & \multirow{3}{*}{TIP}    & \ua{PSNR }              &         & 20.0498 &                          \\
                        &                         & \ua{SSIM }              &         & 0.7153  &                          \\
                        &                         & \da{LPIPS }             &         & 0.2881  &                          \\ \hline
\multirow{6}{*}{TIP}    & \multirow{3}{*}{UHDM}   & \ua{PSNR }              &         & -       &                          \\
                        &                         & \ua{SSIM }              &         & -       &                          \\
                        &                         & \da{LPIPS }             &         & -       &                          \\ \cline{2-6} 
                        & \multirow{3}{*}{FHDMi}  & \ua{PSNR }              &         & -       &                          \\
                        &                         & \ua{SSIM }              &         & -       &                          \\
                        &                         & \da{LPIPS }             &         & -       &                          \\ 
\bottomrule[1.2pt]  % 底部粗线
\end{tabular}
}
\label{tab:Exp_cross_datasets_mbcnn}
\end{table}

==> Tables/tbl_exp_multi_datasets.tex <==
% \begin{table}[t]
% %% Results of the demoireing experiment using the case of multiple dataset training. 
% \caption{Influence of data volume on target dataset TIP~\cite{sun2018moire}.
% %Quantitative results of cross-domain demoireing on the target dataset TIP with incrementally adding new source data. 
% ``F'' represents the FHDMi dataset~\cite{he2020fhde}. ``\dag'' indicates that only natural images are being used.}
% \centering
% % \renewcommand\tabcolsep{5.0pt}
% % \vspace{-8pt}
% % \resizebox{10cm}{!}       % \textwidth, 10cm, 这里用 10cm 好像效果好于 \textwidth
% \scalebox{0.72}
% {       
% \begin{tabular}{ccc|ccc}
% \toprule    % 顶部粗线
% \multirow{2}{*}{Model}    & \multicolumn{2}{c|}{Source Datasets}                        & \multicolumn{3}{c}{Metric}            \\ 
%                                                                                  \cmidrule{2-6} 
%                           & Synthesis             & Demoiréing          & \ua{PSNR } & \ua{SSIM } & \da{LPIPS } \\
% \midrule

% % \multirow{6}{*}{ESDNet-L} & \multirow{5}{*}{UHDM} & UHDM                         &            &            &             \\
% %                           &                       & UHDM + FHDMi\dag {[}25\%{]}  &            &            &             \\
% %                           &                       & UHDM + FHDMi\dag {[}50\%{]}  &            &            &             \\
% %                           &                       & UHDM + FHDMi\dag {[}75\%{]}  &            &            &             \\
% %                           &                       & UHDM + FHDMi\dag {[}100\%{]} &            &            &             \\ 
% %                           \cline{2-6} 
% %                           & UHDM+FHDMi            & UHDM + FHDMi                 &            &            &             \\ 

% \multirow{4}{*}{ESDNet-L} & \multirow{4}{*}{UHDM} & UHDM                     & 19.9983    & 0.7052     & 0.3301      \\
%                           &                       & UHDM + F\dag {[}25\%{]}  & 20.8691    & 0.7491     & 0.2456      \\
%                           % &                       & UHDM + F\dag {[}50\%{]}  & 21.0504    & 0.7579     & 0.2357      \\
%                           &                       & UHDM + F\dag {[}75\%{]}  & 21.0882    & 0.7606     & 0.2245      \\
%                           &                       & UHDM + F\dag {[}100\%{]} & 21.1460    & 0.7672     & 0.2163      \\ 
%                           % \cmidrule{2-6} 
%                           % & UHDM+F                & UHDM + F                 & 21.1558    & 0.7766     & 0.2316      \\ 

% \bottomrule  % 底部粗线
% \end{tabular}
% }
% \label{tab:Exp_multi_datasets}
% % \vspace{-2ex}
% \end{table}


% \begin{table}[t]

% Demoireing results on the UHDM dataset training with synthesized data only. 
% Since both our method and shooting~\cite{shooting} borrow none real moire patterns in dataset UHDM, for fairness, we instruct UnDem~\cite{undem} to utilize the moire patterns from FHDMi~\cite{he2020fhde}. Method "Paired" indicates training using the original real moire data in the training set of UHDM.
% The "C.S." denotes size in the random crop. $(\uparrow)$ denotes the larger, the better, and $(\downarrow)$ denotes the smaller, the better.

%% Quantitative results of cross-domain demoireing on the target dataset TIP with incrementally adding new source data and 1-N synthetic moire pattern 


% \caption{Quantitative results of cross-domain demoireing on the target dataset TIP with 1-N synthetic moire pattern. The ``B'' represents the dataset used in the blending process, and the ``DT'' represents the dataset used in the demoireing training process.}
% \centering
% \renewcommand\tabcolsep{5.0pt}
% \vspace{-8pt}
% % \resizebox{10cm}{!}       % \textwidth, 10cm, 这里用 10cm 好像效果好于 \textwidth
% \scalebox{0.895}
% {       
% % \begin{tabular}{ccc|ccc}
% % \toprule    % 顶部粗线
% % \multirow{2}{*}{Model}    & \multirow{2}{*}{1 to N} & \multirow{2}{*}{Demoireing Training Datasets} & \multicolumn{3}{c}{Metric} \\ \cline{4-6} 
% %                           &                         &                                               &\ua{PSNR }&\ua{SSIM }&\da{LPIPS }   \\ \hline
% % \multirow{8}{*}{ESDNet-L} & \multirow{4}{*}{1 to 1} & UHDM + FHDMi\dag {[}0\%{]}                        &         &        &         \\
% %                           &                         & UHDM + FHDMi\dag {[}25\%{]}                       &         &        &         \\
% %                           &                         & UHDM + FHDMi\dag {[}50\%{]}                       &         &        &         \\
% %                           &                         & UHDM + FHDMi\dag {[}100\%{]}                      &         &        &         \\ 
% %                           \cline{2-6} 
% %                           & \multirow{4}{*}{1 to 3} & UHDM + FHDMi\dag {[}0\%{]}                        &         &        &         \\
% %                           &                         & UHDM + FHDMi\dag {[}25\%{]}                       &         &        &         \\
% %                           &                         & UHDM + FHDMi\dag {[}50\%{]}                       &         &        &         \\
% %                           &                         & UHDM + FHDMi\dag {[}100\%{]}                      &         &        &         \\ 
% % \bottomrule  % 底部粗线
% % \end{tabular}


% % \begin{tabular}{cccc|ccc}
% % \toprule
% % \multirow{2}{*}{Model}     & \multirow{2}{*}{1 to N} & \multicolumn{2}{c|}{Datasets}                        & \multicolumn{3}{c}{Metric} \\ \cline{3-7} 
% %                            &                         & Blending              & Demoireing Training          &\ua{PSNR }&\ua{SSIM }&\da{LPIPS }\\ 
% % %\midrule
% % \hline
% % \multirow{10}{*}{ESDNet-L} & \multirow{5}{*}{1 to 1} & \multirow{4}{*}{UHDM} & UHDM                         &         &        &         \\
% %                            &                         &                       & UHDM + FHDMi\dag {[}25\%{]}  &         &        &         \\
% %                            &                         &                       & UHDM + FHDMi\dag {[}50\%{]}  &         &        &         \\
% %                            &                         &                       & UHDM + FHDMi\dag {[}100\%{]} &         &        &         \\ \cline{3-7} 
% %                            &                         & UHDM+FHDMi            & UHDM + FHDMi                 &         &        &         \\ \cline{2-7} 
% %                            & \multirow{5}{*}{1 to 3} & \multirow{4}{*}{UHDM} & UHDM                         &         &        &         \\
% %                            &                         &                       & UHDM + FHDMi\dag {[}25\%{]}  &         &        &         \\
% %                            &                         &                       & UHDM + FHDMi\dag {[}50\%{]}  &         &        &         \\
% %                            &                         &                       & UHDM + FHDMi\dag {[}100\%{]} &         &        &         \\ \cline{3-7} 
% %                            &                         & UHDM+FHDMi            & UHDM + FHDMi                 &         &        &         \\ 
% % \bottomrule
% % \end{tabular}

% \begin{tabular}{lcc|ccc}
% \toprule
% \multirow{2}{*}{Model}    & \multirow{2}{*}{Datasets (B \& DT)} & \multirow{2}{*}{1 to N} & \multicolumn{3}{c}{Metric}            \\ 
% \cmidrule{4-6} 
%                           &                                  &                         & \ua{PSNR } & \ua{SSIM } & \da{LPIPS } \\
% \midrule
% \multirow{3}{*}{ESDNet-L} & \multirow{3}{*}{UHDM}            & 1 to 1                  & 19.9983    & 0.7052     & 0.3301      \\
%                           &                                  & 1 to 3                  &            &            &             \\
%                           &                                  & 1 to 5                  & 20.5058    & 0.7008     & 0.3292      \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:Exp_1_to_N}
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[h]


% % %Quantitative results of cross-domain demoireing on the target dataset TIP with incrementally adding new source data. 
% % ``F'' represents the FHDMi dataset~\cite{he2020fhde}. ``\dag'' indicates that only natural images are being used.}
% \centering
% \setlength{\tabcolsep}{0.9mm}
% % \scalebox{0.67}
% % {
% % \begin{tabular}{l @{\hskip +0em}|c@{\hskip +2em} c  @{\hskip +2em} c   @{\hskip +2em} c  @{\hskip +2em} c @{\hskip 2em}c}
% \scalebox{0.85}
% {
% \begin{tabular}{l|cccccc}
% \toprule    % 顶部粗线
% % \multicolumn{1}{c}{Method}
% % \multirow{2.5}{*}{Method}
% % \multicolumn{1}{c}{\multirow{2.5}{*}{Method}}
% \multicolumn{1}{c|}{\multirow{2.5}{*}{Method}}    & \multicolumn{3}{c}{UHDM}       & \multicolumn{3}{c}{FHDMi}   \\ 
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
%                            &\ua{PSNR}& \ua{SSIM} & \da{LPIPS}     &\ua{PSNR}& \ua{SSIM} & \da{LPIPS}    \\ 
% % \midrule
% % \multicolumn{7}{c}{\textit{Demoiréing Model: \textbf{ESDNet-L}, trained with \textbf{MHRNID}, 50 Epochs}} \\
% \midrule
% Shooting                   & 10.2568          & 0.5664          & 0.5130          & 11.6022  & 0.5425 & 0.4515  \\
% MoireSpace$\ddagger^{1}$   &           &           &           &   &  &   \\ 
% UnDeM$\dagger$             & 15.2269          & 0.5873          & 0.4190          &          &        &         \\
% UnDeM$\ddagger^{1}$        & 15.2947          & 0.5777          & 0.4241          &          &        &         \\
% \midrule
% Ours$\ddagger^{1}$         & \textbf{17.2524} & \textbf{0.6454} & \textbf{0.3238} & \textbf{19.8128} & \textbf{0.7319} & \textbf{0.2134} \\
% Ours$\ddagger^{3}$         &                  &                 &                 &          &        &         \\ 
% \bottomrule  % 底部粗线
% \end{tabular}
% }
% \caption{Quantitative results of zero-shot demoiréing trained with synthesized data only. ``$\dagger$'', ``$\ddagger^{1}$'' and ``$\ddagger^{3}$'' indicate that the synthetic model is trained with a TIP dataset, a 1-to-1 moiré pattern, and a 1-to-3 moiré pattern. }

% \label{tab:Exp_multi_datasets}
% % \vspace{-2ex}
% \end{table}
		

		


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[ht]
\small
\centering
\setlength{\tabcolsep}{2.7mm}
\scalebox{0.85}{
\begin{tabular}{cc|ccccc|ccccc}
\toprule[1.25pt]
% \multicolumn{2}{c}{Zero   Shot}& \multirow{2.5}{*}{Metric} & \multicolumn{5}{c|}{Demoire Network: MBCNN}  & \multicolumn{5}{c}{Demoire Network:   ESDNet-L}  \\ 
% \cmidrule(lr){1-2} \cmidrule(lr){4-8}  \cmidrule(lr){9-13}

\multirow{2.5}{*}{\makecell{Test \\ Dataset}} & \multirow{2.5}{*}{Metric} & \multicolumn{5}{c|}{Demoiréing Network: \textbf{MBCNN}}  & \multicolumn{5}{c}{Demoiréing Network:   \textbf{ESDNet-L}}  \\ 
 \cmidrule(lr){3-7}  \cmidrule(lr){8-12}
&           & Shooting & UnDeM$^\dagger$ & UnDeM$^\ddagger$ & MoireSpace  & Ours & Shooting & UnDeM$^\dagger$ & UnDeM$^\ddagger$ & MoireSpace & Ours \\ 
\midrule
\midrule
% \multirow{6.5}{*}{MHRNID} 
 \multirow{3}{*}{UHDM}  &\ua{PSNR } & 9.2284  & 13.4256 & 14.5237 & 14.7826 & \textbf{17.9162} & 10.2568 & 15.2269 & 15.2947 & 14.7989 & \textbf{17.2524} \\
                        &\ua{SSIM } & 0.5180  & 0.3973  & 0.4425  & 0.4724  & \textbf{0.6280}  & 0.5664  & 0.5873  & 0.5777  & 0.4859  & \textbf{0.6454}  \\
                        &\da{LPIPS }& 0.6664  & 0.6489  & 0.6332  & 0.5568  & \textbf{0.4162}  & 0.5130  & 0.4190  & 0.4241  & 0.5254  & \textbf{0.3238}  \\ 
\cmidrule{1-12} 
 \multirow{3}{*}{FHDMi} &\ua{PSNR } & 10.6750  & 17.8355 & 18.1652 & 18.5523 & \textbf{19.0094} & 11.6022 & 18.4335 & 18.5390 & 18.0763 & \textbf{19.8128} \\
                        &\ua{SSIM } & 0.4478  & 0.6802  & 0.6999  & 0.7094  & \textbf{0.7137}  & 0.5425  & 0.6900  & 0.6812  & 0.7189  & \textbf{0.7319}  \\
                        &\da{LPIPS }& 0.5978  & 0.2606  & 0.2472  & 0.2742  & \textbf{0.2390}  & 0.4515  & 0.2877  & 0.2986  & 0.2616  & \textbf{0.2134}  \\ 
\bottomrule[1.25pt]
\end{tabular}
}
\caption{Quantitative results of zero-shot demoiréing trained with synthesized data only. 
``$\dagger$'' indicates UnDem uses moiré patterns retrieved from real data in TIP for inference.  ``$\ddagger$''  indicates UnDem uses our generated moiré pattern for inference.
}
\label{tab:Exp_multi_datasets}
\end{table*}










% \begin{table*}[t]
% \small
% \centering
% \setlength{\tabcolsep}{0.9mm}
% \begin{tabular}{ccc|ccccc|ccccc}
% \toprule[1.25pt]
% \multicolumn{2}{c}{Zero   Shot}& \multirow{2.5}{*}{Metric} & \multicolumn{5}{c|}{Demoire Network: MBCNN}  & \multicolumn{5}{c}{Demoire Network:   ESDNet-L}  \\ 
% \cmidrule(lr){1-2} \cmidrule(lr){4-8}  \cmidrule(lr){9-13}
% Source   & Target              &           & Shooting & UnDeM$^\dagger$ & UnDeM$^\ddagger$ & MoireSpace  & Ours & Shooting & UnDeM$^\dagger$ & UnDeM$^\ddagger$ & MoireSpace & Ours \\ 
% \midrule
% \midrule
% \multirow{6.5}{*}{MHRNID} 
% & \multirow{3}{*}{UHDM}  &\ua{PSNR} & 00.0000 & 00.0000 & 00.0000 & 00.0000 & \textbf{00.0000} & 10.2568 & 15.2269 & 15.2947 & 00.0000 & \textbf{17.2524} \\
% &                        &\ua{SSIM} &         &         &         &         &                  & 0.5664  & 0.5873  & 0.5777  &         & \textbf{0.6454}  \\
% &                        &\da{LPIPS}&         &         &         &         &                  & 0.5130  & 0.4190  & 0.4241  &         & \textbf{0.3238}  \\ 
% \cmidrule{2-13} 
% & \multirow{3}{*}{FHDMi} &\ua{PSNR} &         &         &         &         &                  & 11.6022 &         &         &         & \textbf{19.8128} \\
% &                        &\ua{SSIM} &         &         &         &         &                  & 0.5425  &         &         &         & \textbf{0.7319}  \\
% &                        &\da{LPIPS}&         &         &         &         &                  & 0.4515  &         &         &         & \textbf{0.2134}  \\ 
% \bottomrule[1.25pt]
% \end{tabular}
% \caption{Quantitative results of zero-shot demoiréing trained with synthesized data only. 
% ``$\dagger$'' and ``$\ddagger$'' indicate that the UnDem uses real moiré images from TIP or pure moiré patterns for inference.
% }
% \label{tab:Exp_multi_datasets}
% \end{table*}
		
		

